Robust flux error estimation of an unfitted Nitsche method for high-contrast interface problems

We prove an optimal error estimate for the flux variable for a stabilized unfitted Nitsche finite element method applied to an elliptic interface problem with discontinuous constant coefficients. Our result shows explicitly that this error estimate is totally independent of the diffusion coefficients

==> TableErrorsExamplehighcontrastwithJumps.tex <==
\footnotesize
\ra{1.1}
\begin{center}
\begin{tabular}{@{}l@{\hskip .3in}c@{\hskip .2in}c@{\hskip .4in}c@{\hskip .2in}c@{\hskip .4in}c@{\hskip .2in}c@{\hskip .4in}c@{\hskip .2in}c@{}}\toprule
$l$ & $e_h^0$ & eoc & $e_h^\infty$ & eoc  & $e_{h,\rho}^1$ & eoc & $e_{h,\rho}^{1,\infty}$ & eoc \\ \midrule
1   &  1.6e-01  &          &  3.5e-01  &          &   1.3e+04  &         &  2.2e+04 &       \\
2   &  5.2e-02  &   1.66  &  1.2e-01  &   1.50  &   5.8e+03  &  1.22  &  1.4e+04  &  0.72 \\
3   &  1.2e-02  &   2.10  &  3.4e-02  &   1.87  &   2.4e+03  &  1.28  &  6.3e+03  &  1.10 \\
4   &  2.3e-03  &   2.42  &  7.0e-03  &   2.27  &   1.1e+03  &  1.11  &  2.7e+03  &  1.23 \\
5   &  3.7e-04  &   2.62  &  1.3e-03  &   2.45  &   5.4e+02  &  1.03  &  1.2e+03  &  1.13 \\
6   &  6.1e-05  &   2.59  &  2.1e-04  &   2.58  &   2.7e+02  &  1.01  &  5.9e+02  &  1.04 \\
7   &  1.2e-05  &   2.40  &  4.4e-05  &   2.26  &   1.3e+02  &  1.00  &  3.0e+02  &  1.00 \\
 \bottomrule
  \end{tabular}
\end{center}
 \vskip3mm

